Wide and Deep Graph Neural Networks with Distributed Online Learning

Graph neural networks (GNNs) learn representations from network data with naturally distributed architectures, rendering them well-suited candidates for decentralized learning. Oftentimes, this decentralized graph support changes with time due to link failures or topology variations. These changes create a mismatch between the graphs on which GNNs were trained and the ones on which they are tested. Online learning can be used to retrain GNNs at testing time, overcoming this issue. However, most online algorithms are centralized and work on convex problems (which GNNs rarely lead to). This paper proposes the Wide and Deep GNN (WD-GNN), a novel architecture that can be easily updated with distributed online learning mechanisms. The WD-GNN comprises two components: the wide part is a bank of linear graph filters and the deep part is a GNN. At training time, the joint architecture learns a nonlinear representation from data. At testing time, the deep part (nonlinear) is left unchanged, while the wide part is retrained online, leading to a convex problem. We derive convergence guarantees for this online retraining procedure and further propose a decentralized alternative. Experiments on the robot swarm control for flocking corroborate theory and show potential of the proposed architecture for distributed online learning.

==> atNode.tex <==
%!TEX root = ../decentralizedWhitePaper.tex

\def \thisplotscale {0.4}
\def \unit {\thisplotscale cm}

\tikzstyle {block} = [draw,
                      rectangle, 
                      fill = blue!10, 
                      minimum height = 2*\unit]

\tikzstyle {long block}  = [block,
                            minimum width = 4*\unit]

\tikzstyle {short block} = [block,
                            minimum width = 2*\unit]

\tikzstyle {circle block}   = [draw,
                            circle,
                            minimum width = 0.9*\unit]

\def\blockDistance{7}


{\footnotesize\begin{tikzpicture}[x = 1*\unit, y=1*\unit, font=\footnotesize]

% Origin
\node at (0,0) (O) {};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw all blocks
%
% Block for aggregator
\path(O) node (zn) {\includegraphics[width=0.2300\textwidth]{figures/AggregationCNNGSLayer1Input.pdf}};
% Block for CNN
\path (zn.east) ++ (\blockDistance,0) node [long block] (CNN) {CNN};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw all arrows
%
% Arrow into CNN
\path [draw, -stealth] (zn.east) -- (CNN.west)  node  [midway, above] (z) {$\bbz_{i}$};
% Arrow out of CNN
\path [draw, -stealth] (CNN.east) -++ (0.5*\blockDistance,0)  node  [midway,above] (outCNN) {$\bbu_{i}$};


\end{tikzpicture}}




==> graph_convolution.tex <==
% !TEX root = ../decentralizedWhitePaper.tex

\def \thisplotscale {1.8}
\def \unit {\thisplotscale cm}

\tikzstyle {Phi} = [rectangle, 
                    thin,
                    minimum width = 0.5*\unit, 
                    minimum height = \sumshift*\unit, 
                    anchor = west,
                    draw,
                    fill = blue!20]

\tikzstyle {sum} = [circle, 
                    thin,
                    minimum width  = 0.3*\unit, 
                    minimum height = 0.3*\unit, 
                    anchor = center,
                    draw,
                    fill = blue!20]


\def \deltax {2.0}
\def \deltay {0.8}
\def \sumshift {0.4}

\begin{tikzpicture}[x = 1*\unit, y = 1*\unit]
    
% Begin by drawing an empty node for initializing the chain
\node (origin) [] {};
\path (origin) ++ (0.2*\deltax, 0) node (first) [] {};
    
% Draw the chain of graph shifts
\path (first) ++ (1.1*\deltax, 0) node (0) [Phi] {$\bbS$};
\path (0)     ++ (1.0*\deltax, 0) node (1) [Phi] {$\bbS$};
\path (1)     ++ (1.0*\deltax, 0) node (2) [Phi] {$\bbS$};

% End by drawing an empty node for finalizing the chain
\path (2.east) ++ (0.7*\sumshift*\deltax, 0) node [anchor=west] (last) [] {};

% Draw the chain of additions
\path (first.east) ++ (1.5*\sumshift*\deltax, -\deltay) node (sum0) [sum] {$+$};
\path (0.east) ++ (\sumshift*\deltax, -\deltay) node (sum1) [sum] {$+$};
\path (1.east) ++ (\sumshift*\deltax, -\deltay) node (sum2) [sum] {$+$};
\path (2.east) ++ (\sumshift*\deltax, -\deltay) node (sum3) [sum] {$+$};

% Draw the arrows connecting the shift blocks
\path[-stealth] (first) edge [very near start, above] node {$\bbx$}               (0);	
\path[-stealth] (0)     edge [above] node {$\ \bbS\bbx$}     (1);	
\path[-stealth] (1)     edge [above] node {$\ \bbS^{2}\bbx$} (2);	
\path[-]        (2)     edge [above] node {$\ \bbS^{3}\bbx$} (sum3 |- last);

% Draw the arrows connecting to the sum blocks
\path[-stealth, draw] (sum0 |- first) -- (sum0) node [midway, right] {$h_{0}$};	
\path[-stealth, draw] (sum1 |- 0)     -- (sum1) node [midway, right] {$h_{1}$};	
\path[-stealth, draw] (sum2 |- 1)     -- (sum2) node [midway, right] {$h_{2}$};	
\path[-stealth, draw] (sum3 |- 2)     -- (sum3) node [midway, right] {$h_{3}$};

% Draw the arrows connecting the sum blocks
\path[-stealth, draw] (sum0) -- (sum1);	
\path[-stealth, draw] (sum1) -- (sum2);	
\path[-stealth, draw] (sum2) -- (sum3);	

% Draw the convolution output
\path[-stealth] (sum3) edge [above] node 
                {$\bbH(\bbS)\bbx$} ++ (0.4*\deltax, 0);


\end{tikzpicture}
